CCQ: A Multi-State Child Care Quality Dataset to Support AI for Children's Health Research

High-quality child care in early life is a critical determinant of children's growth and development. Research on child care quality has been constrained by fragmented, non-research-friendly, and privacy-bound datasets. We present CCQ (Child Care Quality), a large-scale, de-identified dataset for applied data science research at the intersection of AI and early childhood health. CCQ integrates 59,372 child care provider records across 12 U.S. states, covering diverse provider types as well as data schemas. To ensure research utility while protecting privacy, we implement an automated, LLM-based curation pipeline that anonymizes, cleans, and standardizes raw state records into two complementary releases: a cleaned textual release and a fully preprocessed tabular release. We also benchmark traditional machine learning models, tabular foundation models, and language models on quality rating prediction and important features analytics. Within a state, tabular classifiers on the preprocessed tables perform best. Across states, zero-shot transfer is near chance, but modest target-state supervision recovers most of the within-state performance, and pretraining on other states benefits finetuned language models. We release both datasets with all code to accelerate AI-driven research on child care quality and ultimately improve children's health and development.

==> figs/ccq_fig_kit.tex <==
\edef\ccqEndLine{\the\endlinechar}\endlinechar=-1 \input{figs/model_colors}\endlinechar=\ccqEndLine\relax%
\definecolor{ccqInk}{HTML}{2F3338}%
\definecolor{ccqMute}{HTML}{8A9199}%
\definecolor{ccqLine}{HTML}{B9BFC5}%
\definecolor{ccqLand}{HTML}{E3E6E9}%
\definecolor{ccqZone}{HTML}{F4F6F8}%
\definecolor{ccqData}{HTML}{5A96C4}%
\definecolor{ccqDataLt}{HTML}{D6E6F2}%
\definecolor{ccqTgt}{HTML}{E39B32}%
\definecolor{ccqTgtLt}{HTML}{F8E4C3}%
\definecolor{ccqStar}{HTML}{F2B321}%
\definecolor{ccqHand}{HTML}{5E656D}%
\definecolor{ccqOpen}{HTML}{3E8C5C}%
\definecolor{ccqProp}{HTML}{7A5DA8}%
\definecolor{ccqUp}{HTML}{1A7F45}%
\definecolor{ccqDown}{HTML}{D73027}%
\definecolor{ccqPos}{HTML}{E0806B}%
\definecolor{ccqNeg}{HTML}{6E9FCB}%
\providecommand{\ccqAllStates}{AL,AR,AZ,CA,CO,CT,DC,DE,FL,GA,IA,ID,IL,IN,KS,KY,LA,MA,MD,ME,MI,MN,MO,MS,MT,NC,ND,NE,NH,NJ,NM,NV,NY,OH,OK,OR,PA,RI,SC,SD,TN,TX,UT,VA,VT,WA,WI,WV,WY}%
\def\ccqStateAL{(6.42,-3.84)--(6.89,-3.8)--(7.02,-4.27)--(7.1,-4.4)--(7.06,-4.5)--(7.11,-4.69)--(6.61,-4.74)--(6.66,-4.86)--(6.64,-4.9)--(6.56,-4.88)--(6.53,-4.82)--(6.52,-4.9)--(6.46,-4.89)--(6.42,-4.55)--(6.44,-3.86)--cycle}%
\def\ccqStateAR{(5.23,-3.55)--(5.5,-3.55)--(6.04,-3.52)--(6.05,-3.57)--(6,-3.64)--(6.12,-3.63)--(6.13,-3.67)--(6.05,-3.78)--(6.07,-3.83)--(6.03,-3.87)--(5.98,-3.93)--(5.92,-4.15)--(5.88,-4.2)--(5.89,-4.33)--(5.35,-4.35)--(5.35,-4.23)--(5.26,-4.21)--(5.27,-3.81)--cycle}%
\def\ccqStateAZ{(1.45,-4.07)--(1.49,-4.07)--(1.48,-3.92)--(1.52,-3.89)--(1.54,-3.8)--(1.63,-3.74)--(1.57,-3.56)--(1.6,-3.31)--(1.73,-3.31)--(1.76,-3.13)--(2.39,-3.24)--(2.65,-3.28)--(2.47,-4.56)--(2.08,-4.5)--(1.42,-4.12)--cycle}%
\def\ccqStateCA{(0.33,-1.6)--(1,-1.79)--(0.83,-2.46)--(1.57,-3.56)--(1.63,-3.74)--(1.54,-3.8)--(1.52,-3.89)--(1.48,-3.92)--(1.49,-4.07)--(1.45,-4.07)--(0.99,-4.02)--(0.97,-3.82)--(0.82,-3.62)--(0.7,-3.57)--(0.65,-3.49)--(0.49,-3.44)--(0.46,-3.4)--(0.5,-3.28)--(0.42,-3.13)--(0.35,-2.96)--(0.4,-2.86)--(0.31,-2.74)--(0.33,-2.61)--(0.38,-2.7)--(0.36,-2.57)--(0.29,-2.55)--(0.27,-2.43)--(0.2,-2.29)--(0.24,-2.09)--(0.18,-1.97)--(0.31,-1.73)--cycle}%
\def\ccqStateCO{(2.77,-2.37)--(3.33,-2.44)--(3.61,-2.47)--(3.95,-2.49)--(3.94,-2.72)--(3.9,-3.41)--(3.72,-3.39)--(3.15,-3.34)--(2.65,-3.28)--cycle}%
\def\ccqStateCT{(8.71,-1.84)--(8.99,-1.78)--(9.02,-1.93)--(8.85,-1.98)--(8.74,-2.08)--cycle}%
\def\ccqStateDC{}%
\def\ccqStateDE{(8.45,-2.45)--(8.51,-2.41)--(8.5,-2.44)--(8.55,-2.58)--(8.61,-2.63)--(8.64,-2.7)--(8.53,-2.73)--cycle}%
\def\ccqStateFL{(7.11,-4.69)--(7.14,-4.75)--(7.66,-4.71)--(7.7,-4.76)--(7.69,-4.66)--(7.8,-4.66)--(7.87,-4.86)--(7.95,-5)--(8.06,-5.14)--(8.07,-5.22)--(8.2,-5.44)--(8.23,-5.54)--(8.24,-5.75)--(8.2,-5.86)--(8.07,-5.9)--(8.01,-5.78)--(7.92,-5.75)--(7.85,-5.63)--(7.78,-5.57)--(7.66,-5.43)--(7.71,-5.33)--(7.62,-5.33)--(7.64,-5.17)--(7.59,-5.05)--(7.46,-4.98)--(7.4,-4.91)--(7.27,-4.87)--(7.14,-5.01)--(7.07,-5)--(7.06,-4.94)--(6.96,-4.88)--(6.81,-4.86)--(6.64,-4.9)--(6.66,-4.86)--(6.61,-4.74)--cycle}%
\def\ccqStateGA{(6.89,-3.8)--(7.13,-3.77)--(7.35,-3.74)--(7.32,-3.82)--(7.41,-3.85)--(7.48,-3.96)--(7.71,-4.14)--(7.74,-4.23)--(7.86,-4.35)--(7.83,-4.42)--(7.8,-4.66)--(7.69,-4.66)--(7.7,-4.76)--(7.66,-4.71)--(7.14,-4.75)--(7.11,-4.69)--(7.06,-4.5)--(7.1,-4.4)--(7.02,-4.27)--cycle}%
\def\ccqStateIA{(4.91,-1.95)--(5.49,-1.94)--(5.76,-1.93)--(5.8,-2.11)--(5.87,-2.15)--(5.96,-2.24)--(5.93,-2.36)--(5.82,-2.41)--(5.84,-2.48)--(5.76,-2.65)--(5.71,-2.6)--(5.45,-2.61)--(5.02,-2.62)--(4.97,-2.34)--(4.91,-2.18)--(4.88,-2.12)--cycle}%
\def\ccqStateID{(1.71,-1.02)--(1.71,-0.92)--(1.84,-0.36)--(1.98,-0.39)--(1.93,-0.62)--(1.95,-0.74)--(2.01,-0.8)--(2.09,-0.96)--(2.13,-0.96)--(2.05,-1.2)--(2.15,-1.18)--(2.19,-1.39)--(2.24,-1.42)--(2.25,-1.49)--(2.37,-1.48)--(2.56,-1.54)--(2.47,-2.1)--(1.98,-2.01)--(1.49,-1.91)--(1.58,-1.5)--(1.62,-1.43)--(1.57,-1.37)--(1.76,-1.12)--cycle}%
\def\ccqStateIL{(5.76,-2.65)--(5.84,-2.48)--(5.82,-2.41)--(5.93,-2.36)--(5.96,-2.24)--(5.87,-2.15)--(6.34,-2.12)--(6.4,-2.3)--(6.47,-2.98)--(6.38,-3.17)--(6.39,-3.2)--(6.39,-3.27)--(6.32,-3.3)--(6.32,-3.37)--(6.24,-3.34)--(6.21,-3.4)--(6.14,-3.33)--(6.14,-3.26)--(5.98,-3.13)--(6.01,-2.98)--(5.91,-2.97)--(5.9,-2.9)--(5.78,-2.8)--cycle}%
\def\ccqStateIN{(6.4,-2.3)--(6.52,-2.28)--(6.86,-2.24)--(6.86,-2.25)--(6.93,-2.84)--(6.94,-2.92)--(6.83,-2.95)--(6.74,-3.13)--(6.69,-3.09)--(6.55,-3.19)--(6.47,-3.15)--(6.39,-3.2)--(6.38,-3.17)--(6.47,-2.98)--cycle}%
\def\ccqStateKS{(3.94,-2.72)--(4.65,-2.75)--(5.1,-2.75)--(5.16,-2.78)--(5.14,-2.86)--(5.22,-2.95)--(5.23,-3.44)--(4.89,-3.44)--(4.33,-3.43)--(3.9,-3.41)--cycle}%
\def\ccqStateKY{(6.21,-3.4)--(6.24,-3.34)--(6.32,-3.37)--(6.32,-3.3)--(6.39,-3.27)--(6.39,-3.2)--(6.47,-3.15)--(6.55,-3.19)--(6.69,-3.09)--(6.74,-3.13)--(6.83,-2.95)--(6.94,-2.92)--(6.93,-2.84)--(6.99,-2.83)--(7.04,-2.9)--(7.21,-2.92)--(7.27,-2.88)--(7.33,-2.95)--(7.34,-3.02)--(7.41,-3.11)--(7.47,-3.13)--(7.35,-3.25)--(7.29,-3.34)--(7.2,-3.39)--(7.04,-3.41)--(6.45,-3.46)--(6.41,-3.5)--(6.17,-3.51)--cycle}%
\def\ccqStateLA{(5.35,-4.35)--(5.89,-4.33)--(5.91,-4.45)--(5.95,-4.48)--(5.84,-4.67)--(5.83,-4.79)--(6.19,-4.77)--(6.18,-4.85)--(6.25,-4.95)--(6.19,-4.99)--(6.27,-5.07)--(6.26,-5.13)--(6.32,-5.14)--(6.34,-5.22)--(6.2,-5.15)--(6.13,-5.21)--(6.08,-5.15)--(6.01,-5.23)--(5.9,-5.17)--(5.84,-5.08)--(5.79,-5.06)--(5.71,-5.13)--(5.54,-5.08)--(5.41,-5.1)--(5.43,-5.02)--(5.42,-4.9)--(5.45,-4.76)--(5.35,-4.58)--cycle}%
\def\ccqStateMA{(8.71,-1.68)--(8.84,-1.65)--(9.03,-1.61)--(9.09,-1.55)--(9.14,-1.58)--(9.09,-1.66)--(9.22,-1.78)--(9.31,-1.77)--(9.2,-1.83)--(9.18,-1.79)--(9.13,-1.86)--(9.11,-1.83)--(9.1,-1.82)--(9.05,-1.76)--(8.99,-1.78)--(8.71,-1.84)--cycle}%
\def\ccqStateMD{(7.82,-2.57)--(8.45,-2.45)--(8.53,-2.73)--(8.64,-2.7)--(8.63,-2.8)--(8.55,-2.84)--(8.52,-2.85)--(8.46,-2.71)--(8.39,-2.66)--(8.42,-2.52)--(8.37,-2.54)--(8.36,-2.69)--(8.44,-2.84)--(8.35,-2.82)--(8.27,-2.74)--(8.28,-2.7)--(8.26,-2.67)--(8.14,-2.6)--(8.05,-2.53)--(8,-2.58)--(7.94,-2.57)--(7.84,-2.69)--cycle}%
\def\ccqStateME{(9.1,-1.5)--(9.05,-1.45)--(8.91,-1.02)--(9,-0.86)--(8.99,-0.67)--(9.06,-0.48)--(9.12,-0.52)--(9.23,-0.46)--(9.3,-0.5)--(9.39,-0.8)--(9.45,-0.8)--(9.46,-0.87)--(9.52,-0.88)--(9.57,-0.95)--(9.5,-1.06)--(9.36,-1.18)--(9.31,-1.1)--(9.3,-1.23)--(9.18,-1.31)--(9.13,-1.38)--cycle}%
\def\ccqStateMI{(6.52,-2.28)--(6.59,-2.16)--(6.59,-1.98)--(6.52,-1.84)--(6.52,-1.75)--(6.55,-1.6)--(6.64,-1.48)--(6.74,-1.42)--(6.7,-1.38)--(6.75,-1.33)--(6.97,-1.4)--(7.01,-1.47)--(7.02,-1.62)--(6.94,-1.77)--(6.99,-1.8)--(7.05,-1.71)--(7.1,-1.68)--(7.15,-1.72)--(7.22,-1.91)--(7.21,-2)--(7.16,-1.99)--(7.08,-2.22)--(6.86,-2.25)--(6.86,-2.24)--cycle (5.85,-1.23)--(6.01,-1.16)--(6.19,-1.01)--(6.24,-1)--(6.15,-1.12)--(6.28,-1.14)--(6.33,-1.21)--(6.44,-1.21)--(6.52,-1.15)--(6.7,-1.11)--(6.7,-1.18)--(6.83,-1.15)--(6.84,-1.21)--(6.94,-1.28)--(6.74,-1.31)--(6.63,-1.27)--(6.38,-1.4)--(6.32,-1.53)--(6.27,-1.47)--(6.28,-1.4)--(6.23,-1.35)--(5.9,-1.28)--cycle}%
\def\ccqStateMN{(4.79,-0.71)--(5.11,-0.71)--(5.11,-0.62)--(5.16,-0.64)--(5.2,-0.77)--(5.4,-0.78)--(5.63,-0.87)--(5.66,-0.91)--(5.77,-0.86)--(5.96,-0.91)--(5.82,-0.98)--(5.59,-1.19)--(5.6,-1.21)--(5.56,-1.22)--(5.56,-1.36)--(5.48,-1.47)--(5.51,-1.5)--(5.49,-1.66)--(5.72,-1.82)--(5.76,-1.93)--(5.49,-1.94)--(4.91,-1.95)--(4.91,-1.54)--(4.84,-1.47)--(4.89,-1.4)--(4.86,-1.23)--(4.85,-1.02)--(4.81,-0.89)--cycle}%
\def\ccqStateMO{(5.02,-2.62)--(5.45,-2.61)--(5.71,-2.6)--(5.76,-2.65)--(5.78,-2.8)--(5.9,-2.9)--(5.91,-2.97)--(6.01,-2.98)--(5.98,-3.13)--(6.14,-3.26)--(6.14,-3.33)--(6.21,-3.4)--(6.17,-3.51)--(6.16,-3.51)--(6.15,-3.52)--(6.12,-3.63)--(6,-3.64)--(6.05,-3.57)--(6.04,-3.52)--(5.5,-3.55)--(5.23,-3.55)--(5.23,-3.44)--(5.22,-2.95)--(5.14,-2.86)--(5.16,-2.78)--(5.1,-2.75)--cycle}%
\def\ccqStateMS{(5.89,-4.33)--(5.88,-4.2)--(5.92,-4.15)--(5.98,-3.93)--(6.03,-3.87)--(6.42,-3.84)--(6.44,-3.86)--(6.42,-4.55)--(6.46,-4.89)--(6.36,-4.9)--(6.25,-4.95)--(6.18,-4.85)--(6.19,-4.77)--(5.83,-4.79)--(5.84,-4.67)--(5.95,-4.48)--(5.91,-4.45)--cycle}%
\def\ccqStateMT{(1.98,-0.39)--(2.65,-0.52)--(3.03,-0.57)--(3.4,-0.62)--(3.77,-0.66)--(3.71,-1.34)--(3.69,-1.56)--(3.39,-1.53)--(2.98,-1.48)--(2.58,-1.42)--(2.56,-1.54)--(2.37,-1.48)--(2.25,-1.49)--(2.24,-1.42)--(2.19,-1.39)--(2.15,-1.18)--(2.05,-1.2)--(2.13,-0.96)--(2.09,-0.96)--(2.01,-0.8)--(1.95,-0.74)--(1.93,-0.62)--cycle}%
\def\ccqStateNC{(7.56,-3.34)--(7.8,-3.31)--(8.12,-3.26)--(8.59,-3.16)--(8.59,-3.23)--(8.47,-3.33)--(8.63,-3.29)--(8.66,-3.35)--(8.6,-3.44)--(8.43,-3.43)--(8.54,-3.47)--(8.5,-3.56)--(8.59,-3.54)--(8.56,-3.61)--(8.44,-3.65)--(8.34,-3.77)--(8.33,-3.84)--(8.23,-3.86)--(7.98,-3.68)--(7.78,-3.71)--(7.72,-3.65)--(7.49,-3.67)--(7.35,-3.74)--(7.13,-3.77)--(7.13,-3.71)--(7.21,-3.63)--(7.26,-3.62)--(7.38,-3.5)--(7.51,-3.46)--cycle}%
\def\ccqStateND{(3.77,-0.66)--(4.45,-0.7)--(4.79,-0.71)--(4.81,-0.89)--(4.85,-1.02)--(4.86,-1.23)--(4.89,-1.4)--(4.6,-1.39)--(4.12,-1.37)--(3.71,-1.34)--cycle}%
\def\ccqStateNE{(3.65,-2.01)--(4.04,-2.04)--(4.57,-2.06)--(4.66,-2.12)--(4.76,-2.1)--(4.91,-2.18)--(4.97,-2.34)--(5.02,-2.62)--(5.1,-2.75)--(4.65,-2.75)--(3.94,-2.72)--(3.95,-2.49)--(3.61,-2.47)--cycle}%
\def\ccqStateNH{(8.86,-1.11)--(8.91,-1.02)--(9.05,-1.45)--(9.1,-1.5)--(9.09,-1.55)--(9.03,-1.61)--(8.84,-1.65)--(8.81,-1.46)--(8.82,-1.28)--(8.88,-1.22)--cycle}%
\def\ccqStateNJ{(8.49,-2.46)--(8.5,-2.44)--(8.51,-2.41)--(8.61,-2.31)--(8.5,-2.21)--(8.5,-2.14)--(8.55,-2.04)--(8.7,-2.09)--(8.69,-2.16)--(8.69,-2.17)--(8.67,-2.21)--(8.71,-2.22)--(8.73,-2.37)--(8.65,-2.57)--(8.49,-2.46)--cycle}%
\def\ccqStateNM{(2.65,-3.28)--(3.15,-3.34)--(3.72,-3.39)--(3.72,-3.51)--(3.71,-3.51)--(3.63,-4.53)--(2.95,-4.47)--(2.96,-4.52)--(2.64,-4.48)--(2.63,-4.58)--(2.47,-4.56)--cycle}%
\def\ccqStateNV{(1,-1.79)--(1.49,-1.91)--(1.98,-2.01)--(1.76,-3.13)--(1.73,-3.31)--(1.6,-3.31)--(1.57,-3.56)--(0.83,-2.46)--cycle}%
\def\ccqStateNY{(7.68,-2)--(7.8,-1.86)--(7.75,-1.76)--(7.84,-1.72)--(8,-1.72)--(8.09,-1.69)--(8.19,-1.61)--(8.15,-1.46)--(8.2,-1.41)--(8.32,-1.24)--(8.58,-1.18)--(8.62,-1.34)--(8.64,-1.49)--(8.67,-1.5)--(8.71,-1.68)--(8.71,-1.84)--(8.74,-2.08)--(9,-2.02)--(8.86,-2.13)--(8.72,-2.19)--(8.69,-2.16)--(8.7,-2.09)--(8.55,-2.04)--(8.5,-2.02)--(8.41,-1.92)--(7.69,-2.06)--cycle}%
\def\ccqStateOH{(6.86,-2.25)--(7.08,-2.22)--(7.26,-2.27)--(7.38,-2.23)--(7.48,-2.13)--(7.56,-2.09)--(7.61,-2.39)--(7.58,-2.63)--(7.46,-2.73)--(7.44,-2.83)--(7.41,-2.8)--(7.38,-2.93)--(7.33,-2.95)--(7.27,-2.88)--(7.21,-2.92)--(7.04,-2.9)--(6.99,-2.83)--(6.93,-2.84)--cycle}%
\def\ccqStateOK{(3.72,-3.39)--(3.9,-3.41)--(4.33,-3.43)--(4.89,-3.44)--(5.23,-3.44)--(5.23,-3.55)--(5.27,-3.81)--(5.26,-4.21)--(5.12,-4.13)--(4.99,-4.15)--(4.92,-4.2)--(4.81,-4.14)--(4.76,-4.19)--(4.67,-4.13)--(4.54,-4.09)--(4.52,-4.11)--(4.24,-3.98)--(4.26,-3.54)--(3.72,-3.51)--cycle}%
\def\ccqStateOR{(0.71,-0.7)--(0.8,-0.8)--(0.79,-0.87)--(0.86,-0.91)--(0.98,-0.91)--(1.03,-0.95)--(1.39,-0.95)--(1.71,-1.02)--(1.76,-1.12)--(1.57,-1.37)--(1.62,-1.43)--(1.58,-1.5)--(1.49,-1.91)--(1,-1.79)--(0.33,-1.6)--(0.33,-1.4)--(0.45,-1.21)--(0.57,-0.92)--(0.65,-0.71)--cycle}%
\def\ccqStatePA{(7.56,-2.09)--(7.68,-2)--(7.69,-2.06)--(8.41,-1.92)--(8.5,-2.02)--(8.55,-2.04)--(8.5,-2.14)--(8.5,-2.21)--(8.61,-2.31)--(8.51,-2.41)--(8.45,-2.45)--(7.82,-2.57)--(7.65,-2.6)--(7.61,-2.39)--cycle}%
\def\ccqStateRI{(9.02,-1.93)--(8.99,-1.78)--(9.05,-1.76)--(9.1,-1.82)--(9.08,-1.91)--cycle}%
\def\ccqStateSC{(7.35,-3.74)--(7.49,-3.67)--(7.72,-3.65)--(7.78,-3.71)--(7.98,-3.68)--(8.23,-3.86)--(8.16,-3.92)--(8.14,-4.04)--(8.01,-4.19)--(7.92,-4.24)--(7.86,-4.35)--(7.74,-4.23)--(7.71,-4.14)--(7.48,-3.96)--(7.41,-3.85)--(7.32,-3.82)--cycle}%
\def\ccqStateSD{(3.69,-1.56)--(3.71,-1.34)--(4.12,-1.37)--(4.6,-1.39)--(4.89,-1.4)--(4.84,-1.47)--(4.91,-1.54)--(4.91,-1.95)--(4.88,-2.12)--(4.91,-2.18)--(4.76,-2.1)--(4.66,-2.12)--(4.57,-2.06)--(4.04,-2.04)--(3.65,-2.01)--cycle}%
\def\ccqStateTN{(6.12,-3.63)--(6.15,-3.52)--(6.16,-3.51)--(6.17,-3.51)--(6.41,-3.5)--(6.45,-3.46)--(7.04,-3.41)--(7.2,-3.39)--(7.56,-3.34)--(7.51,-3.46)--(7.38,-3.5)--(7.26,-3.62)--(7.21,-3.63)--(7.13,-3.71)--(7.13,-3.77)--(6.89,-3.8)--(6.42,-3.84)--(6.03,-3.87)--(6.07,-3.83)--(6.05,-3.78)--(6.13,-3.67)--cycle}%
\def\ccqStateTX{(3.72,-3.51)--(4.26,-3.54)--(4.24,-3.98)--(4.52,-4.11)--(4.54,-4.09)--(4.67,-4.13)--(4.76,-4.19)--(4.81,-4.14)--(4.92,-4.2)--(4.99,-4.15)--(5.12,-4.13)--(5.26,-4.21)--(5.35,-4.23)--(5.35,-4.35)--(5.35,-4.58)--(5.45,-4.76)--(5.42,-4.9)--(5.43,-5.02)--(5.41,-5.1)--(5.22,-5.17)--(5.24,-5.09)--(5.18,-5.11)--(5.2,-5.19)--(5.1,-5.3)--(4.92,-5.39)--(4.8,-5.48)--(4.77,-5.47)--(4.69,-5.64)--(4.68,-5.76)--(4.71,-5.92)--(4.74,-5.95)--(4.52,-5.92)--(4.34,-5.84)--(4.28,-5.7)--(4.28,-5.59)--(4.12,-5.41)--(4.05,-5.22)--(3.9,-5.06)--(3.66,-5.05)--(3.57,-5.22)--(3.37,-5.11)--(3.3,-5.04)--(3.28,-4.92)--(3.23,-4.8)--(3.16,-4.75)--(2.96,-4.52)--(2.95,-4.47)--(3.63,-4.53)--(3.71,-3.51)--cycle}%
\def\ccqStateUT{(1.98,-2.01)--(2.47,-2.1)--(2.44,-2.32)--(2.77,-2.37)--(2.65,-3.28)--(2.39,-3.24)--(1.76,-3.13)--cycle}%
\def\ccqStateVA{(8.55,-2.84)--(8.63,-2.8)--(8.58,-2.88)--(8.57,-3.01)--(8.53,-3.01)--cycle (7.47,-3.13)--(7.5,-3.19)--(7.61,-3.18)--(7.77,-3.09)--(7.84,-2.83)--(7.9,-2.86)--(7.94,-2.75)--(7.97,-2.77)--(8.03,-2.66)--(8.03,-2.59)--(8.13,-2.65)--(8.14,-2.6)--(8.26,-2.67)--(8.28,-2.7)--(8.27,-2.74)--(8.25,-2.79)--(8.46,-2.87)--(8.49,-3.05)--(8.46,-3.1)--(8.55,-3.08)--(8.59,-3.16)--(8.12,-3.26)--(7.8,-3.31)--(7.56,-3.34)--(7.2,-3.39)--(7.29,-3.34)--(7.35,-3.25)--cycle}%
\def\ccqStateVT{(8.58,-1.18)--(8.86,-1.11)--(8.88,-1.22)--(8.82,-1.28)--(8.81,-1.46)--(8.84,-1.65)--(8.71,-1.68)--(8.67,-1.5)--(8.64,-1.49)--(8.62,-1.34)--cycle}%
\def\ccqStateWA{(1.84,-0.36)--(1.71,-0.92)--(1.71,-1.02)--(1.39,-0.95)--(1.03,-0.95)--(0.98,-0.91)--(0.86,-0.91)--(0.79,-0.87)--(0.8,-0.8)--(0.71,-0.7)--(0.64,-0.65)--(0.67,-0.51)--(0.66,-0.23)--(0.7,-0.2)--(0.77,-0.27)--(0.9,-0.33)--(0.97,-0.39)--(0.92,-0.52)--(0.96,-0.52)--(1.02,-0.38)--(1.02,-0.21)--(1,-0.14)--(1.4,-0.25)--cycle}%
\def\ccqStateWI{(5.6,-1.21)--(5.76,-1.15)--(5.85,-1.23)--(5.9,-1.28)--(6.23,-1.35)--(6.28,-1.4)--(6.27,-1.47)--(6.32,-1.53)--(6.28,-1.66)--(6.42,-1.48)--(6.35,-1.65)--(6.35,-1.74)--(6.31,-1.95)--(6.34,-2.12)--(5.87,-2.15)--(5.8,-2.11)--(5.76,-1.93)--(5.72,-1.82)--(5.49,-1.66)--(5.51,-1.5)--(5.48,-1.47)--(5.56,-1.36)--(5.56,-1.22)--cycle}%
\def\ccqStateWV{(7.33,-2.95)--(7.38,-2.93)--(7.41,-2.8)--(7.44,-2.83)--(7.46,-2.73)--(7.58,-2.63)--(7.61,-2.39)--(7.65,-2.6)--(7.82,-2.57)--(7.84,-2.69)--(7.94,-2.57)--(8,-2.58)--(8.05,-2.53)--(8.14,-2.6)--(8.13,-2.65)--(8.03,-2.59)--(8.03,-2.66)--(7.97,-2.77)--(7.94,-2.75)--(7.9,-2.86)--(7.84,-2.83)--(7.77,-3.09)--(7.61,-3.18)--(7.5,-3.19)--(7.47,-3.13)--(7.41,-3.11)--(7.34,-3.02)--cycle}%
\def\ccqStateWY{(3.69,-1.56)--(3.65,-2.01)--(3.61,-2.47)--(3.33,-2.44)--(2.77,-2.37)--(2.44,-2.32)--(2.47,-2.1)--(2.56,-1.54)--(2.58,-1.42)--(2.98,-1.48)--(3.39,-1.53)--cycle}%
\def\ccqOffCA{(-0.91,2.84)}%
\def\ccqOffCO{(-3.30,2.89)}%
\def\ccqOffGA{(-7.38,4.25)}%
\def\ccqOffKY{(-6.81,3.17)}%
\def\ccqOffMD{(-8.23,2.65)}%
\def\ccqOffMT{(-2.85,0.97)}%
\def\ccqOffNC{(-7.89,3.51)}%
\def\ccqOffNE{(-4.36,2.38)}%
\def\ccqOffOK{(-4.49,3.80)}%
\def\ccqOffSC{(-7.77,4.00)}%
\def\ccqOffWA{(-1.24,0.58)}%
\def\ccqOffWI{(-5.95,1.64)}%
\providecommand{\ccqUSMap}[2]{%
  \begin{scope}[#1]\begin{scope}[shift={(-4.878,3.048)}]%
    \foreach \s in \ccqAllStates {\fill[ccqLand, draw=white, line width=0.3pt] \csname ccqState\s\endcsname;}%
    \foreach \s/\c in {#2}{\fill[\c, draw=white, line width=0.3pt] \csname ccqState\s\endcsname;}%
  \end{scope}\end{scope}}%
\providecommand{\ccqStateAt}[4]{%
  \begin{scope}[shift={#2}, scale=#3]%
    \edef\ccqTmp{\noexpand\begin{scope}[shift={\csname ccqOff#1\endcsname}]}\ccqTmp
    \path[#4] \csname ccqState#1\endcsname;%
  \end{scope}\end{scope}}%
\tikzset{
  who/.style={circle, fill=#1, text=white, minimum size=9.5pt, inner sep=0pt,
               font=\fontsize{5.6}{5.6}\selectfont},
  station/.style={circle, draw=ccqInk, fill=white, line width=0.7pt, minimum size=0.80cm,
               inner sep=0pt, font=\fontsize{12}{12}\selectfont},
  pics/ccq raw/.style={code={%
    \draw[ccqInk!55, fill=white, line width=0.4pt, rounded corners=0.8pt]
      (-0.52,-0.37) rectangle (0.64,0.50);
    \draw[ccqInk, fill=white, line width=0.5pt, line join=round]
      (-0.62,-0.46) -- (-0.62,0.41) -- (0.35,0.41) -- (0.54,0.22) -- (0.54,-0.46) -- cycle;
    \draw[ccqInk, line width=0.4pt, line join=round] (0.35,0.41) -- (0.35,0.22) -- (0.54,0.22);
    \node[text=ccqInk, font=\fontsize{6.2}{6.2}\selectfont] at (-0.43,0.22) {\faIcon{school}};
    \draw[ccqInk, line width=1.0pt, line cap=round] (-0.27,0.23) -- (0.18,0.23);
    \foreach \y/\l in {0.03/0.92, -0.11/0.72, -0.25/0.84}{%
      \draw[ccqMute, line width=0.55pt, line cap=round] (-0.49,\y) -- ++(\l,0);}
    \node[text=ccqStar, font=\fontsize{4.1}{4.1}\selectfont] at (0.10,-0.375)
      {\faIcon{star}\faIcon{star}\faIcon{star}\faIcon[regular]{star}\faIcon[regular]{star}};
  }},
  pics/ccq prep/.style={code={%
    \draw[ccqInk!55, fill=white, line width=0.4pt, rounded corners=0.8pt]
      (-0.52,-0.37) rectangle (0.64,0.50);
    \fill[white] (-0.62,-0.46) rectangle (0.54,0.41);
    \fill[ccqLand] (-0.62,0.235) rectangle (0.54,0.41);
    \fill[ccqStar!22] (0.25,-0.46) rectangle (0.54,0.235);
    \foreach \x in {-0.33,-0.04,0.25}{\draw[ccqLine, line width=0.35pt] (\x,-0.46) -- (\x,0.41);}
    \foreach \y in {0.235,0.06,-0.115,-0.29}{\draw[ccqLine, line width=0.35pt] (-0.62,\y) -- (0.54,\y);}
    \draw[ccqInk, line width=0.5pt] (-0.62,-0.46) rectangle (0.54,0.41);
    \node[text=ccqStar, font=\fontsize{4.6}{4.6}\selectfont] at (0.395,0.322) {\faIcon{star}};
    \foreach \r/\a/\b/\c/\d in {0.147/1/0/24/3, -0.028/0/1/12/5, -0.203/1/1/60/2, -0.375/0/0/8/4}{%
      \node[text=ccqInk, font=\sffamily\fontsize{4.3}{4.3}\selectfont] at (-0.475,\r) {\a};
      \node[text=ccqInk, font=\sffamily\fontsize{4.3}{4.3}\selectfont] at (-0.185,\r) {\b};
      \node[text=ccqInk, font=\sffamily\fontsize{4.3}{4.3}\selectfont] at (0.105,\r) {\c};
      \node[text=ccqInk, font=\sffamily\bfseries\fontsize{4.3}{4.3}\selectfont] at (0.395,\r) {\d};}
  }},
  pics/ccq folds/.style={code={%
    \foreach \i in {0,...,4}{%
      \fill[ccqDataLt, draw=white, line width=0.5pt] (0,0) -- (90-\i*72:0.2) arc (90-\i*72:18-\i*72:0.2) -- cycle;}
    \fill[ccqTgt, draw=white, line width=0.5pt] (0,0) -- (90:0.2) arc (90:18:0.2) -- cycle;
  }},
  pics/ccq bars/.style={code={%
    \foreach \x/\h/\c in {-0.30/0.20/LR, -0.12/0.44/RF, 0.06/0.34/XGB, 0.24/0.52/MBERT, 0.42/0.30/LoRA}{%
      \filldraw[fill=c\c!50, draw=c\c, line width=0.4pt] (\x-0.065,-0.26) rectangle (\x+0.065,-0.26+\h);
      \draw[ccqInk, line width=0.35pt] (\x,-0.26+\h-0.05) -- (\x,-0.26+\h+0.05);}
    \draw[ccqInk, line width=0.45pt] (-0.46,0.33) -- (-0.46,-0.26) -- (0.54,-0.26);
  }},
  pics/ccq shap/.style={code={%
    \foreach \y/\v in {0.24/0.46, 0.12/-0.34, 0.0/0.27, -0.12/0.19, -0.24/-0.12}{%
      \ifdim\v pt>0pt\def\ccqc{ccqUp}\else\def\ccqc{ccqDown}\fi
      \filldraw[fill=\ccqc!50, draw=\ccqc, line width=0.4pt] (0.02,\y-0.042) rectangle (0.02+\v,\y+0.042);}
    \draw[ccqInk, line width=0.45pt] (0.02,0.33) -- (0.02,-0.33);
  }},
  pics/ccq curve/.style={code={%
    \draw[ccqInk, line width=0.45pt] (-0.46,0.33) -- (-0.46,-0.26) -- (0.54,-0.26);
    \draw[ccqTgt, line width=0.8pt, line join=round]
      (-0.34,-0.17) -- (-0.14,0.06) -- (0.06,0.16) -- (0.26,0.22) -- (0.46,0.25);
    \foreach \x/\y in {-0.34/-0.17, -0.14/0.06, 0.06/0.16, 0.26/0.22, 0.46/0.25}{%
      \filldraw[fill=white, draw=ccqTgt, line width=0.5pt] (\x,\y) circle (0.035);}
  }},
}%


==> figs/model_colors.tex <==
\definecolor{cDummy}{HTML}{A3A19B}
\definecolor{cLR}{HTML}{FAB72A}
\definecolor{cRF}{HTML}{0FCBDB}
\definecolor{cXGB}{HTML}{7A8AF6}
\definecolor{cTabPFN}{HTML}{C35AA4}
\definecolor{cTabNN}{HTML}{D16022}
\definecolor{cMBERT}{HTML}{84CEFE}
\definecolor{cCORN}{HTML}{8747D7}
\definecolor{cCLS}{HTML}{4AD186}
\definecolor{cRAG}{HTML}{7C9128}
\definecolor{cLoRA}{HTML}{FAA9C1}

